A Radiative Transfer Framework for Spatially-Correlated Materials

We introduce a non-exponential radiative framework that takes into account the local spatial correlation of scattering particles in a medium. Most previous works in graphics have ignored this, assuming uncorrelated media with a uniform, random local distribution of particles. However, positive and negative correlation lead to slower- and faster-than-exponential attenuation respectively, which cannot be predicted by the Beer-Lambert law. As our results show, this has a major effect on extinction, and thus appearance. From recent advances in neutron transport, we first introduce our Extended Generalized Boltzmann Equation, and develop a general framework for light transport in correlated media. We lift the limitations of the original formulation, including an analysis of the boundary conditions, and present a model suitable for computer graphics, based on optical properties of the media and statistical distributions of scatterers. In addition, we present an analytic expression for transmittance in the case of positive correlation, and show how to incorporate it efficiently into a Monte Carlo renderer. We show results with a wide range of both positive and negative correlation, and demonstrate the differences compared to classic light transport.

==> src25_overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%!TEX root = src00_main.tex

\section{Overview}
\label{sec:overview}
\diego{consider removing the section and taking it to the end of intro?}

We will first present a general background of radiative transport in correlated media, a brief summary of the effect of spatial correlation on Extinction, and the Generalized Boltzmann Equation (GBE, \Sec{RTCM}). 
Unfortunately, this equation is not suitable for rendering, due to its strong simplifying assumptions. In \Sec{ourgbe} we will present our extended GBE, which lifts the limitations of the original GBE to support more general media, and include a thorough analysis of its boundary conditions. 
Finally, in \Sec{local_optical_parameters} we propose a practical formulation for appearance of positively correlated media based on local optical parameters, which is intuitive and easy to manipulate, and which can be plugged directly into our extended GBE. 
%\diego{complete roadmap once fixed}

==> src30_background.tex <==
%!TEX root = src00_main.tex

\section{Background: The Radiative Transport Equation}
\label{sec:background}

Light transport in participating media is modeled by the radiative transfer equation (RTE)~\cite{Chandrasekhar1960}.
%, which is a form of the Boltzmann linear transport equation. 
In its integro-differential form it models the directional derivative of flux $\sRad$ at point $\px$ as:
\begin{equation}
\diro\cdot\Diff{\sRad(\px,\diro)} + \sExtinction\sRad(\px,\diro) = \sRadI(\px,\diro) + \sEmission(\px,\diro),
\label{eq:rte}
\end{equation}
%
where $\sEmission(\diro)$ is the volume source term, and $\sRadI$ is the in-scattered radiance:
\begin{equation}
\sRadI(\px,\diro) = \sScattering\int_\Sphere \sRad(\px,\diri)\sPF(\px,\diri,\diro)\diff{\diri},
\label{eq:inscattering}
\end{equation}
which is the directional integral in the sphere $\Sphere$ of the light scattered towards $\diro$, modeled using the phase function $\sPF$; $\diri$ represents the incoming direction of light. Note that we have omitted the spatial dependency of all terms in \Eqs{rte}{inscattering} for simplicity.
%
Finally, $\sExtinction=\sAbsorption+\sScattering$ in \si{\per\meter} is the extinction coefficient, with $\sAbsorption$ and $\sScattering$ the absorption and scattering coefficients respectively. These terms model the probability of a beam of light to be attenuated either by absorption or scattering, and are defined as the product of the number of particles per unit volume $\sConcentration$ (\si{\per\cubic\meter}), and the particles' cross section $\sCrossSection$ (\si{\square\meter}), assuming that the particles are uniformly distributed in the differential volume (\Fig{isotropic_dragons}, left). 

Jakob et al.~\shortcite{Jakob2010Radiative} later generalized the RTE to model directionally anisotropic media, by taking into account the angular (directional) dependence of the particle's cross sections in media such as wood, hair or cloth. This anisotropy transforms \Eqs{rte}{inscattering} into:
%
\begin{align}
&\diro\cdot\Diff{\sRad(\diro)} + \sExtinction(\diro)\sRad(\diro) = \sRadI(\diro) + \sEmission(\diro), \label{eq:anisrte} \\
&\sRadI(\diro) = \sScattering(\diro)\int_\Sphere \sRad(\diri)\sPF(\diri,\diro)\diff{\diri}.
\label{eq:anisinscattering}
\end{align}
%
The main difference with respect to $\Eq{rte}$ is that the extinction $\sExtinction(\diro)$ and scattering $\sScattering(\diro)$ coefficients, as well as the phase function $\sPF(\diri,\diro)$, now dependent on the particles' directional distribution probability $\sProbDir{\dir}$ as:
\begin{align}
&\sExtinction(\diro) = \sConcentration \int_\Sphere \sCrossSection(\diro,\dir)\sProbDir{\dir}\diff{\dir}, \label{eq:extinction_jakob}\\
&\sScattering(\diro) = \sConcentration \int_\Sphere \sAlbedo(\diro,\dir)\sCrossSection(\diro,\dir) \sProbDir{\dir} \diff{\dir}, \nonumber \\
&\sPF(\diri,\diro) = \frac{\sConcentration}{\sScattering(\diro)} \int_\Sphere \sPF(\diri,\diro,\dir)\sAlbedo(\diro,\dir)\sCrossSection(\diro,\dir)\sProbDir{\dir}\diff{\dir}, \nonumber
\end{align}
%
where $\sCrossSection(\diro,\dir)$ and  $\sAlbedo(\diro,\dir)$ are respectively the projected area and the scattering albedo of a particle oriented towards $\dir$ in direction $\diro$, and $\sPF(\diri,\diro,\dir)$ is the phase function of particles oriented towards $\dir$. 

Jakob's form of the RTE still assumes that the particles are distributed uniformly in the \emph{spatial} domain, i.e., it assumes perfect decorrelation in their positions. In the following, we relax this assumption and generalize the RTE to \textit{locally correlated} media.
%where the positions of the particles present correlation, 
This requires a reformulation of the extinction and scattering coefficients, and therefore of the full radiative model, for which we leverage recent advances in transport theory.
%, introducing in graphics the Generalized Boltzmann Equation~\cite{Larsen2007Generalized,Larsen2011Generalized} \diego{check: nobody had used it before in CG?}; we then 
%extending them to support directionally structured and anisotropic media. 



==> src40_structured_rte.tex <==
%!TEX root = src00_main.tex
\section{Radiative Transport in Correlated Media}
\label{sec:srte}

\adrianc{Rev on Nov 22} \diego{to be detailed and finished after Sec. 4 is done. Skipping for now}
In this section we first introduce the notion of spatial correlation in media, and its effect on light extinction (\Sec{sec:correlation}). We then introduce the Generalized Boltzmann Equation (GBE), proposed by Larsen~\shortcite{Larsen2007Generalized} in the context of neutron transport (\Sec{larsengbe}). We 
show how Larsen's original formulation is not suitable for rendering due to its strong limitations, and modify the GBE to support more general media as existing in rendering (\Sec{ourgbe}), including a thorough analysis of boundary conditions (\Sec{boundary_conditions}). 


It is important to first clarify the difference between spatially-correlated media, and heterogenous media, as commonly used in computer graphics. As illustrated in \Fig{heterogenous_vs_correlated}, heterogeneous media assume \textit{local} homogeneity at each differential volume $\vV(\px)$. In contrast, correlated media takes into account the average effect of uneven particle distributions within each $\vV(\px)$. Therefore, a medium can be \emph{statistically homogeneous}, meaning that its statistical moments are invariant over all the volume, but spatially correlated~\cite{Kostinski2001Extinction}. 

\begin{figure}
  \def\svgwidth{.99\columnwidth}
\footnotesize
  \input{images/rte/correlated_vs_heterogeneous/correlated_vs_heterogeneous.pdf_tex}
\caption{Distinction between heterogeneous and spatially-correlated media. Heterogeneous media assume heterogeneity at a macroscopic level, but local homogeneity at each differential volume $\vV(\px)$ (represented as solid colors per voxel). Instead, spatially-correlated media takes into account the uneven distribution of particles within each $\vV(\px)$ (represented as probability functions).}
\label{fig:heterogenous_vs_correlated}
\end{figure}

%In this section, we first introduce the theory of spatially-correlated media, arriving at the Generalized Boltzmann Equation (GBE). We then  develop a particular formulation of such equation which is suitable for rendering, thus making the theory usable in computer graphics. \adrianc{We need to make our contriubutions here more explicty!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
\centering
  \def\svgwidth{.99\columnwidth}
  \input{images/rte/correlation/correlation.pdf_tex}
%
\caption{\diego{this figure is not referenced until late in the paper; why is it here again?} 
Illustration of the effect of spatial correlation in a medium. (a) A random distribution of particles within a differential volume $\vV(\px)$. (b) In the presence of particle correlation, the probability of interaction changes within $\vV(\px)$. (c, d) This correlation might further exhibit directional behavior, leading to very different interaction probabilities according to the degree of alignment with the propagation of light. 
%Illustration of the effect of spatial correlation. For media with a random distribution of particles (a) the distribution of particles within a differential volume $\vV(\px)$ is uniform.  In the presence of particle correlation, the probability of an interaction changes within a differential volume $\vV(\px)$ (b).   
%This correlation might further exhibit directional behavior: in these cases, if the direction of correlation is aligned to the direction of light propagation, the probability of traversing $\vV(\px)$ undisturbed might be very high (c). In contrast, if the direction of correlation is orthogonal (d) to the propagation of light, the effect of correlation disappears, and the probability of extinction is statistically similar to the uniform distribution assumed by the classic RTE. 
}
\label{fig:correlation}
\end{figure}
%

\subsection{\new{Effect of Spatial Correlation on Extinction}}
\label{sec:correlation}
When light propagates through a participating medium, it scatters as a function of the distribution of the scattering particles. When this distribution is random, extinction becomes a Poissonian process, and the exponential Beer-Lambert law accurately describes the attenuation of light (see~\cite{Gallavotti1972} for a rigorous derivation). However, the distribution of particles in many media exhibit different forms and degrees of spatial correlation (e.g. clouds~\cite{Lovejoy1995,Davis2004Photon}, textiles~\cite{Coquard2006}, porous materials~\cite{Bellet2009,Taine2010}, or granular aggregates~\cite{Meng2015Granular}). As a consequence, attenuation is no longer exponential, and light extinction becomes non-Poissonian.

\new{Negative correlation occurs when the distribution of particles is more uniform than Poisson (as in electrostatic repulsion), and leads to super-exponential (faster) extinction. Clustered particles, on the other hand, yield positive correlation, which leads to sub-exponential (slower) extinction; this is illustrated in \Fig{pos_neg}. \diego{We have skipped Fig. 4!}}
%
\new{The reason for such non-exponential transmittance can be intuitively visualized in \Fig{kostinskis}: In negatively-correlated media, absorbers are  less likely to "shadow" one another; as a result, more light becomes extinct. Positively-correlated media presents the opposite case, with many absorbers shadowing others; this creates empty regions which in turn lead to more light passing through.} 



\begin{figure}
\includegraphics[width=\columnwidth]{images/schematic_views/correlation}
\caption{\new{Different types of particle correlation, and their effect on transmittance. From left to right, the first three figures depict negative correlation, no correlation (extinction is a Poissonian process), and positive correlation. The plot on the right shows extinction: While uncorrelated media results in the classic exponential extinction, negative and positive correlation lead to faster- and slower-than-exponential extinction, respectively. \diego{the positive correlation shows this only for long distances, but first it shows much less transmittance. I'm not sure we want to show this; can we produce cleaner plots, without this effect (or at least not so exaggerated) since this is just for illustration?}}}
\label{fig:pos_neg}
\end{figure}
%
\begin{figure}
  \def\svgwidth{.99\columnwidth}
\footnotesize
  \input{images/schematic_views/kostinski_attenuation.pdf_tex}
%\includegraphics[width=\columnwidth]{images/schematic_views/kostinski_attenuation}
\caption{\new{Intuitive explanation for non-exponential transmittance in negatively- (left) and positively-correlated (right) media. Solid squares represent perfect absorbers. Although both media have the same number of absorbers, shadowing (or overlapping) of such particles (positive correlation) results in less (sub-exponential) extinction. Figure inspired from~\cite{Kostinski2002}.}}
\label{fig:kostinskis}
\end{figure}


%Simple distribution examples for super- and sub-exponential extinction, where particles have negative (left) and positive (right) correlation, respectively. Solid squares indicate perfect absorbers; both media have the same number of extincting particles. In the super-exponential case the obstacles are enforced to not be aligned in the propagation direction (negative correlation), while in the sub-exponential case they tend to follow the opposite approach, tending to alignment in the propagation direction (positive correlation). This different correlations have a large impact on the amount of light passing through the media: in negatively correlated media it is more likely to find an extincting particle, so less light passes through. In contrast, positively correlated particles are more likely to shadow each other, and therefore less light beams will be occluded, resulting in more light passing through. Figure inspired from~\cite{Kostinski2002}.}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new{More formally, in uncorrelated media (Poissonian process) the extinction probability after traveling a distance $t$ from the previous scattering (or emission\footnote{We will refer only to scattering events from now on for simplicity.}) event is $\sProb{t}=\sExtinction\,\exp(-\sExtinction\,t)$, as predicted by the Beer-Lambert law. Thus, defining the differential probability of extinction $\sExtinctionResolved(t)$ [\si{\per\meter}] as
%
\begin{equation}
\sExtinctionResolved(t) = \frac{\sProb{t}}{1-\int_0^t\sProb{s}\diff{s}},
\label{eq:extinctionresolved}
\end{equation}
%
we obtain $\sExtinctionResolved(t) = \sExtinction$, the extinction coefficient of the media (uniform for each differential volume, and independent of the distance $t$).}

\new{Let us now define a simple positively correlated (clustered) medium, composed of regions with a high density of particles (extinction coefficient $\sExtinctionIdx{1}$), and regions with low density ($\sExtinctionIdx{2}$). The probability of light extinction after traveling a distance $t$ is given by~\cite{Larsen2011Generalized}
%
\begin{equation}
\sProb{t} = \sExtinctionIdx{1}\,\sProbExt{\sExtinctionIdx{1}}\,e^{-\sExtinctionIdx{1}\,t} + \sExtinctionIdx{2}\,\sProbExt{\sExtinctionIdx{2}}\,e^{-\sExtinctionIdx{2}\,t},
\label{eq:prob_two_extinction}
\end{equation}
%
with $\sProbExt{\sExtinctionIdx{1}}$ and $\sProbExt{\sExtinctionIdx{2}}$ the probability of traversing a region with extinction coefficients $\sExtinctionIdx{1}$ and $\sExtinctionIdx{2}$ respectively, where $\sProbExt{\sExtinctionIdx{1}}+\sProbExt{\sExtinctionIdx{2}} = 1$.
From this simple example, we can see that $\sProb{t}$ is not exponential anymore, and extinction is no longer a Poissonian process with a constant $\sExtinctionResolved(t) = \sExtinction$. Instead, plugging  \Eq{prob_two_extinction} into \Eq{extinctionresolved} leads to a function dependent on $t$. In other words, spatial correlation introduces a \emph{memory effect}, where the differential probability of extinction depends on the traveled distance $t$ since the previous scattering event. This has a significant effect in the final volumetric appearance of the medium, as shown in \Fig{isotropic_dragons}. \diego{add all other final results where this can be seen}}

%\diego{What happened to the awesome figure by Kostinski that we loved so much?} \adrianc{I'm planning to add that in Sec. 5.} \diego{maybe (we'll see) a forward reference: this will be used in Sec 5....}




%\begin{comment}
%As we have seen, in correlated media the exponential attenuation predicted by the Beer-Lambert law does not hold. Instead, assuming for now isotropic correlation, the extinction probability of a photon becomes a function of the distance $t$ traveled since the previous scattering (or emission\footnote{We will refer only to scattering events from now on for simplicity.}) event~\cite{Larsen2011Generalized}. 
%\new{Let $\sExtinctionResolved(t)$ [\si{\per\meter}] be the average differential probability that a photon will be extinguished after traveling a distance $t$ in direction $\diro$:
%%
%\begin{equation}
%\sExtinctionResolved(t) = \frac{\sProb{t}}{1-\int_0^t\sProb{s}\diff{s}},
%\label{eq:extinctionresolved}
%\end{equation}
%%
%with $\sProb{t}$ [\si{\per\meter}] the probability of extinction at distance $t$ after the last scattering event. Note that when $\sProb{t}$ is exponential as predicted by the classic RTE \ParEq{rte}, then $\sExtinctionResolved(t)$ becomes constant. \adrianc{Is this a good time to make the differences between $\sExtinctionResolved(t)$ and $\sExtinction$ explicit? Maybe it'd be good to relate them using the example in \Eq{prob_two_extinction}? I think this would answer \RevTF}.} \diego{if you're asking... then yes. In general, we need to spoon-feed this paper to the reviewers, even if some parts end up in supp. }
%\diego{this is the unused but maybe useful text (needs rewording): }To describe this more formally, let us take a simple example of two media (extinctions $\sExtinctionIdx{1}$ and $\sExtinctionIdx{2}$) combining to made up one heterogeneous medium. The probability of extinction after traveling a distance $t$ is
%%
%\begin{equation}
%\sProb{t} = \sExtinctionIdx{1}\,\sProbExt{\sExtinctionIdx{1}}\,e^{-\sExtinctionIdx{1}\,t} + \sExtinctionIdx{2}\,\sProbExt{\sExtinctionIdx{2}}\,e^{-\sExtinctionIdx{2}\,t},
%\label{eq:prob_two_extinction}
%\end{equation}
%%
%with $\sProbExt{\sExtinctionIdx{1}}$ and $\sProbExt{\sExtinctionIdx{2}}$ the probability of finding extinction coefficient $\sExtinctionIdx{1}$ and $\sExtinctionIdx{2}$ respectively, holding $\sProbExt{\sExtinctionIdx{1}}+\sProbExt{\sExtinctionIdx{2}} \leq 1$.
%Even in this very simple example, it is easy to see that $\sProb{t}$ is not the classic exponential probability, as we detail in \Sec{srte}.
%% \adrianc{\cite[Fig.1]{Kostinski2002} is awesome for showing this! It shows an example for negative correlation, but could also be used to example positive correlation (and no correlation); moreover, it EXACTLY shows what our definition of media (based on \sProb{\sConcentration}) means!. The question is whether use it for showing also $\sScatteringResolved(t)$, because the type of correlation might be a bit different (what \RevFS means is correlation in the sense of \cite[Fig.2]{Kostinski2002}; we also mean so, but more locally and related with something like \cite[Fig.1]{Kostinski2002}.}
%This has a significant effect in the final volumetric appearance, as shown in \Fig{isotropic_dragons}. 
%\adrianc{End copied text}
%\end{comment}


\subsection{Generalized Boltzmann Equation}
\label{sec:larsengbe}
\new{Since $\sExtinctionResolved(t)$ is a function of $t$ in the presence of correlation, flux $\sRad(\px,\diro)$ now becomes $\sRad(\px,\diro,t)$, the flux at $\px$ after traveling a distance $t$ from the last scattering event. This in turn introduces an additional derivative term in \Eq{rte}, resulting in the \emph{Generalized Boltzmann Equation} (GBE)~\cite{Larsen2007Generalized,Larsen2011Generalized} (see \diego{Appendix XX} for the full derivation):} %\diego{I'm still having trouble figuring out where previous works end and our contribution begins}\adrianc{Does the new intro of Sec.4 helps? Now I say that explicitly.}:
%
\begin{multline}
\frac{d}{dt}\sRad(\px,\diro,t) + \diro\cdot\Diff{\sRad(\px,\diro,t)} + \sExtinctionResolved(t)\sRad(\px,\diro,t) = 0, \\
\sRad(\px,\diro,0) = \underbrace{\int_0^\infty\sScatteringResolved(t)\int_\Sphere \sRad(\px,\diri,t)\sPF(\diri,\diro)\diff{\diri}\diff{t}}_{\text{Inscattering $\sRadI(\px,\diro)$}} + \sEmission(\px,\diro),
\label{eq:larsengrte}
\end{multline}
%
where \new{$\sScatteringResolved(t)=\sAlbedo\,\sExtinctionResolved(t)$} is the probability of a particle being scattered after traveling a distance $t$. \new{The second line of the equation represents the initial value for $t=0$, in which light is scattered or emitted. Thus, after each scattering event the memory effect for the extinction is reset to zero. 
}

Note that by removing the $t$-dependency as $\sExtinctionResolved(t) = \sExtinctionResolved$, and integrating \Eq{larsengrte}, we obtain the classic RTE defined by \Eq{rte}, as expected \new{\diego{(see Appendix XXX)}}. 
%
\new{Moreover, \Eq{larsengrte} can also support directionally anisotropic media~\cite{Jakob2010Radiative} by formulating $\sExtinctionResolved$ as a function of $\diro$~\cite{Vasques2014anisotropic}}. 

\new{Unfortunately, \Eq{larsengrte} relies on a set of simplifying assumptions, which make it unsuitable for rendering applications. In particular~\cite{Larsen2007Generalized,Larsen2011Generalized}}\footnote{Larsen and Vasques also assume that the system is monoenergetic (single wavelength), and the introduction of $\sExtinctionResolved(t)$. Removing the former is straightforward, while the second has already been introduced when deriving \Eq{extinctionresolved}.}:
%\diego{cite Larsens paper. Also, we discussed this before but I forgot what we agreed on: Larsen mentions five limitations, and that's probably what the reviewers will want to see here. Why only three?}: 
%
\new{\begin{enumerate}
\item The medium is statistically homogeneous, and infinite, so that all its optical properties, as well as its differential probability of extinction $\sExtinctionResolved(t)$, are independent of the position in space. No system boundaries exist. 
 \item The phase function $\sPF(\diri,\diro)$ and albedo $\sAlbedo$ are independent of $t$. This means that there is no spatial correlation between $\sPF$ and $\sAlbedo$, which might not be true when dealing with real-world volumetric appearance.  For example, in a mixture of two types of particles with different phase function or albedo, this assumes that both types have the exact same correlation or structure. 
% , which in many cases (e.g. volumetric level-of-detail) might not be true. 
\item The source term $\sEmission(\px,\diro)$ is correlated with the rest of particles in the volume. This assumption will obviously not hold in most cases. 
% isotropic, and satisfies that $\sEmission(\px)\rightarrow 0$ as $|\px|\rightarrow \infty$. This implies that all the medium is emissive, with power decreasing as a function of distance from its center. 
 \end{enumerate}
%
}
In order to make the GBE useful for rendering, we need to generalize it further, lifting these three assumptions. The next section describes this, introducing our novel, extended GBE.

%\diego{same problem as before: if we keep citing papers, what is our contribution? Not clear where PW ends and we begin}\adrianc{Our contribution, up to this point, is to realize that structured material exist in rendering, that most previous work don't do it right, and for handling this we need to rely in other forms of RTE (in particular, the proposed by Larsen, and its anisotropic extension). }

%\adrianc{Need to talk about the $t$-dependence on the phase function $\sPF$ and the scattering albedo $\sAlbedo$, that results on mixing a bunch of different scatterers with (potentially) different spatial distributions (i.e. different measures of correlation); this is a contribution wrt previous work on correlated media (Larsen and so on), generalizing the GBE to account for this $t$-dependence. }
%\adrianc{Should we write the assumptions of Larsen (infinite homogeneous media) somewhere here? The thing is that these assumptions can be broken even within \Eq{larsengrte}, by imposing locality on $\sExtinctionResolved(t)$ and on the rest of optical properties. }

%\begin{comment}
%Except for a few works that solve the RTE in its differential form~\cite{Gutierrez2005,Munoz2014,Ament2014}, in graphics it is generally evaluated in its integral form. Solving the ordinal differential equation (ODE) defined in \Eq{grte} for the radiance incoming at point $\px$ we get:
%% Extending Larsen and Vasques's integral definition~\cite{Larsen2011Generalized} to support heterogeneous media, 
%%
%%\adrianc{I'd like to revise this once more: \cite{Larsen2011Generalized} modeled only their equation for homogeneous media, as well as others such as Davis~\cite{Davis2004Photon,Davis2014Generalized}. I have the (internal) proofs for the homogeneous case; but I'd like to be sure that this heterogeneous formulation is rock solid...}. 
%%
%%
%\begin{equation}
%\sRad(\diro) = \int_0^\infty \underbrace{e^{-\int_{0}^{t}\sExtinctionResolved(s)\diff{s}}}_{\sTranmittanceCorr(\px,\px_t)} \left(\sRadICorr(\px_t,\diro) + \sEmission(\px_t,\diro)\right)\diff{t},
%\label{eq:integral_grte}
%\end{equation}
%%
%where $\px_t = \px - \diro\,t$, and $\sExtinctionResolved(s)$ is defined locally at point $\px_t$. \adrianc{As \RevFS states, \Eq{integral_grte} assumes correlation between $\sEmission$ and the scatterers, which essentially mean that emitting particles have the same distribution as scattering/absorbing particles in the media (i.e. they are correlated). While this might be true in some cases, this is definitely not true for e.g. a point light source in the media. In that case, the transmittance $\sTranmittanceCorr$ would be different between $\sRadICorr$ and $\sEmission$, due to different correlation with the media. Also, as noted in \cite{Ament2014}, $\sEmission$ should be multiplied by the absorption, which itself might be (or not) correlated with the media.} The term $\sTranmittanceCorr(\px,\px_t)$ represents the transmittance between points $\px$ and $\px_t$, while the inscattering $\sRadICorr(\px_t,\diro)$ is
%%
%\begin{equation}
%\sRadICorr(\px_t,\diro) = \int_0^\infty\sScatteringResolved(t')\int_\Sphere \sRad(\px_{t'},\diri)\sTranmittanceCorr(\px_t,\px_{t'})\sPF(\diri,\diro,t')\diff{\diri}\diff{t'},
%\label{eq:integral_inscattering}
%\end{equation}
%%
%\new{where $\px_{t'}=\px_t+\diri\,t'$.} Once again, note that $\sScatteringResolved(t')$ is defined locally in $\px_t$ \adrianc{\RevTF and \RevEE asked us for a figure illustrating the what we mean by each thing in this integral (similar to the usual figure showing participating media. We can add it...}
%\end{comment}



==> src45_rendering_extended_GBE.tex <==
%!TEX root = src00_main.tex
\subsection{\new{Using the Extended GBE}}
\label{sec:ggbe_rendering}
\new{
%
%
Up to this point, we have extended Larsen's original GBE formulation~\ParEq{larsengrte}, lifting the assumptions that made it unsuitable for rendering \ParEq{grteours}
%{grteoursinitial_source}
presenting it also in integral form \ParEq{integral_grte}.
%{integral_inscattering}
Our extended GBE  supports an arbitrary mixture of scatterers (see \App{mixtures}), heterogeneous media, and accounts for the effect of different correlation between scatterers and sources. 
%
The required differential extinction probabilities can be precomputed by sampling the media and tabulating the averaged extinction probabilities; this is the approach used in previous works~\cite{Moon2007Discrete,Larsen2011Generalized,Frank2010Generalized}, for the case of the original GBE. Alternatively, an empirical $\sProb{t}$ can be used. In both cases, $\sExtinctionResolved(\px,t)$ is computed by inverting $\sProb{t}$ via \Eq{extinctionresolved}.
%Alternatively, an empirical free path distribution can be used. In both cases, $\sExtinctionResolved(\px,t)$ is computed by inverting the free path distribution via \Eq{extinctionresolved}.
%
}
\new{
Unfortunately, an explicit connection with the optical parameters of the media, commonly used in rendering, does not exist with this formulation. 
Our new model described in \Sec{local_optical_parameters} overcomes this, providing the missing connection.
}

%\adrianc{Note to future Adrian: It'd be very cool to render a media with arbitrary free path distributions (e.g. Cauchy or Weibull)! Maybe we can add some specific $\sProb{t}$ and their sampling procedures in the supp material, or just refer to d'Eon's Hitchhicker's guide, or diffusion papers.}
%\Eqs{integral_grte}{integral_inscattering} define the appearance of the media based on the differential extinction probabilities $\sExtinctionResolvedI{\sRadI}(\px,t)$ and $\sExtinctionResolvedI{\sEmission_j}(\px,t)$, as well as their associated scattering operators $\sScatteringOperator_{\sRadI}(\px,\diri,\diro,t)$ and $\sScatteringOperator_{\sEmission_j}(\px,\diri,\diro,t)$. Unfortunately, computing each of them is not as direct as in the classic RTE where the differential probability of extinction is the same for both the particle-to-particle scattering and the source terms and is constant $\sExtinctionResolved(\px,t)=\sExtinction$. 
%
%In the case of generalized transport, we cannot directly compute $\sExtinctionResolved(\px,t)$ from the optical of the media; instead, the common approach~\cite{Moon2007Discrete,Larsen2011Generalized,Frank2010Generalized} is to precompute the free path distribution \diego{wrong macro?} $\sProb(t)$ via explicit simulations, and then compute $\sExtinctionResolved(\px,t)$ using \Eq{extinctionresolved}. Other (theoretical) alternative consists on defining an analytic free path distribution $\sProb(t)$, although this distribution might not necessarily represent the path length of any existing correlated media. Note also that in the case of arbitrary free path distributions the relationship between $\sExtinctionResolvedI{\sRadI}(\px,t)$ and $\sExtinctionResolvedI{\sEmission_j}(\px,t)$ needs to be defined. 
%



%\adrianc{Key: This model is general, supports every media (from correlation -1 to 1), and any path length distribution. The prob is that you need to either tabulate, or make up the $\sProb{t}$. In the next section, we develop a model under certain assumptions (correlation smaller than $dt$, positive correlation), that works in most media used in graphics (except for granular materials), but that can be defined using optical properties, and that is efficient as hell}

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\adrianc{To do (empirical analysis is being carried out, plus we're deriving some theory for that. For now, just copied some of the 2.2 rev comments to have them fresh.}

\emph{\begin{displayquote}[\cite{Frank2010Generalized}]
"Second, the theory in this paper must be extended to finite media. For such problems, boundary conditions for the nonclassical angular flux on the outer boundary of the system must be formulated in a way that is consistent with standard outer boundary conditions to the relevant diffusion approximation. Specifically, what should the assigned value of s be for particles that enter the system from the exterior? The choice s = 0 is intuitively appealing but is not necessarily correct." 
\end{displayquote}}

\emph{\begin{displayquote}
``Regarding memory: it makes perfect sense to me in an infinite medium that from correlation stats you can come up with non-exponential free-path transport that better describes what is going on, but if the memory between scattering events is so significant, as you show and claim, what about the memory at boundaries? If you reflect off a boundary and the cluster of particles you just scattered from is very close or was very far, shouldn't your extinction after the reflection be very different in both cases if you roughly hit the wall/mirror normally? And how do the statistics change if you hit at grazing angles and as you strike the medium from the outside. Is it even possible to maintain the correlated distribution up to the boundary, and how do you even measure that? What if you cross a dielectric boundary between two media with slightly different (or even identical) homogeneous locally-correlated properties inside? Is your t value reset to 0 or carried through the refraction? This was an element that I feel Moon et al. 2007 got wrong with their spherical shell accelerators: they reset t to 0 at the surface of each sphere despite not colliding with the correlated particles. ``
\end{displayquote}}


==> src50_structured_local_rte_Adrian.tex <==
%!TEX root = src00_main.tex
%\section{Radiative Transport in Correlated Media}

\section{Modeling Correlated Media from Optical Parameters}
\label{sec:local_optical_parameters}
\new{In this section we move from our extended, general formulation of light transport in correlated media described so far, to a model where the parameters are defined locally, based on the optical parameters of the media, and an statistical description of the structure created by correlation. }

%\new{As discussed in \Sec{ggbe_rendering}, the $t$-dependent average differential probabilities of extinction \diego{have we dropped the x?}$\sExtinctionResolved(t)$ cannot be directly computed directly from the primal optical properties of the media as in the uncorrelated RTE (e.g. the extinction coefficient $\sExtinctionResolved(t)=\sExtinction=\sConcentration\,\sCrossSection$). 
%%
%Unfortunately, using the primal optical parameters has obvious advantages allowing for more intuitive direct definition of the media, as well as editing its optical properties locally. }
\begin{figure}
  \def\svgwidth{.99\columnwidth}
%\footnotesize
  \input{images/schematic_views/kostinski_same_distance.pdf_tex}
%\includegraphics[width=\columnwidth]{images/schematic_views/kostinski_attenuation}
\caption{\new{Examples of three differential volumes in a medium, each with different distribution on the light direction of propagation, but with similar distribution of particles on the plane perpendicular to the direction of propagation, in a simple media similar to the shown in \Fig{kostinskis}. In our model \ParEq{transmittance} the three volumes are modeled with the same probability distribution of optical depths $\sProbExtinction{\sExtinction}$. }\adrianc{Edit the fig to illustrate $\sBeamFront$!} }
\label{fig:kostinskis_differential}
\end{figure}
%
\new{Let us first return to the effect of correlation over extinction, as illustrated in \Fig{kostinskis}: As light traverses a correlated medium, it is attenuated according to the distribution of particles. 
%
Assuming that correlation occurs in a differential volume, and thus the scale of correlation is smaller than a differential distance $\diff{t}$, then the exact position of the particles within the volume becomes irrelevant; only their projection onto the plane perpendicular to the direction of propagation (i.e. the beam propagation front $\sBeamFront$) \diego{not a big fan of this font...} matters (see \Fig{kostinskis_differential}). 
%
As we will show in this section, this insight will allow us to define extinction from the optical properties of the medium. 
%
This is different from granular media~\cite{Moon2007Discrete}, where the correlation distance is larger than $\diff{t}$ and in the scale (or larger) than the granular particle's size. The consequence is that the probability of extinction $\sProb{t}$ is not necessarily monotonically decreasing, making the distribution of particles along the propagation direction relevant, so that the explicit path length distribution needs to be taken into account. %Despite this limitation, as we will see it will allow for a simpler definition of the media, which is still general enough for graphics applications. 
}

\new{Under this assumption, we can compute the total light passing through a distance $t$ on a correlated medium $\sRad_o(t)$ as the integral of the attenuated light at each differential ray of the beam propagation front $\sBeamFront$. Defining the attenuation function of the ray $\sRay\in\sBeamFront$ as $\sAttenuation(\sOpticalDepth_t(\sRay))$, a function of the optical depth $\sOpticalDepth_t(\sRay)$ at distance $t$, and the input radiance at ray $\sRay$ as $\sRad_i(\sRay)$, then $\sRad_o(t)$ is
%
\begin{align}
\sRad_o(t) & =  \int_\sBeamFront \sRad_i(\sRay) \,\sAttenuation(\sOpticalDepth_t(\sRay)) \diff{\sRay}.
\label{eq:light_transmitted_general_spatial}
\end{align}
%
Note that we have used a generic attenuation function $\sAttenuation(\sOpticalDepth_t(\sRay))$; if the particles distribution is random (although correlated) then the extinction at each differential ray of the beam is Poissonian, holding $\sAttenuation(\sOpticalDepth_t(\sRay))=e^{-\sOpticalDepth_t(\sRay)}$. In other cases, in particular in ordered (deterministic) media presenting negative correlation, this attenuation does not hold. We elaborate on that later in \Sec{attenuation}, but for now we stick to the generic $\sAttenuation(\sOpticalDepth_t(\sRay))$. 
%
Also, by using the assumptions of arbitrary particles position on the direction of propagation and small propagation distance $t$ we can simplify the optical depth to the homogeneous case where $\sOpticalDepth_t(\sRay)=\sExtinction(\sRay)\,t$. This will allow us to simplify notation in the following. }
%

\new{Explicitly integrating over all rays of the beam propagation front is not practical. Instead, we would like to find a compact way of relating $\sRad_i(\sRay)$ with the extinction coefficient $\sExtinction(\sRay)$ driving attenuation. We can remove the spatial dependence on ray $\sRay$ by modeling the incoming light as a distribution $\sProbLight{\sRad_i}$, and explicitly relating the light distribution with the extinction coefficient $\sExtinction$ with a conditional distribution $\sProbExtinctionConditional{\sExtinction}{\sRad_i}$. By doing so, and using $\hat{\sRad}_i=\int_\sBeamFront \sRad_i(\sRay)\diff{\sRay}$ we transform \Eq{light_transmitted_general_spatial} into
%
\begin{align}
\sRad_o(t)& = \hat{\sRad}_i \int_0^\infty \int_0^\infty \sProbLight{\sRad_i}\, \sProbExtinctionConditional{\sExtinction}{\sRad_i} \, \sAttenuation(\sExtinction \,t ) \,\diff{\sExtinction}\,\diff{\sRad_i}.
\label{eq:light_transmitted_general}
\end{align}
%
Finally, by using the definition of transmittance as $\sTranmittanceCorr(t)=\frac{\sRad_o(t)}{\hat{\sRad}_i}$ then we get
%
\begin{align}
\sTranmittanceCorr(t) = \int_0^\infty \int_0^\infty \sProbLight{\sRad_i}\, \sProbExtinctionConditional{\sExtinction}{\sRad_i} \, \sAttenuation(\sExtinction \,t ) \, \diff{\sExtinction}\,\diff{\sRad_i}.
\label{eq:transmittance_general}
\end{align}
%
}

\new{Then, from \Eq{transmittance_general} we can compute the probability of extinction $\sProb{t}$ as
\begin{align}
\sProb{t} = \left|\frac{\diff{\sTranmittanceCorr(t)}}{\diff{t}}\right| = \int_0^\infty \int_0^\infty \sProbLight{\sRad_i}\, \sProbExtinctionConditional{\sExtinction}{\sRad_i} \, \left|\frac{\diff{\sAttenuation(\sExtinction \,t )}}{\diff{t}}\right| \, \diff{\sExtinction}\,\diff{\sRad_i}.
\label{eq:pathlength_dist_general}
\end{align}
%
Finally, $\sExtinctionResolved(t)$ can be directly computed from $\sProb{t}$ using \Eq{extinctionresolved}. }

\new{\Eqs{transmittance_general}{pathlength_dist_general} are general, and can model any type of correlation on the plane $\sBeamFront$, including both positive and negative correlations. In particular, the effect of positive correlation is handled by the particular distribution of extincting particles in the media $\sProbExtinctionConditional{\sExtinction}{\sRad_i}$. In contrast, negative correlation manifests on the attenuation function $\sAttenuation(\sExtinction \,t)$, breaking the stochastic nature of the extinction for individual rays $\sRay\in\sBeamFront$. This means that one media could be negatively correlated on $\sBeamFront$ at a low scale, but the particules could be still positively correlated at higher levels, stressing the multiscale behaviour of extinction on correlated media, already discussed by Kostinski~\shortcite{Kostinski2001Extinction,Kostinski2002}. In the following, we discuss in more depth the implications of \Eq{light_transmitted_general}, and elaborate on a practical special case from which we build our model for rendering in \Sec{rendering}.}


\subsection{The attenuation function $\sAttenuation(\sExtinction \,t)$}
%
\label{sec:attenuation}
\new{As discussed earlier, the term $\sAttenuation(\sExtinction \,t)$ models the type of extinction suffered for an individual ray. This is dependent on the particular distribution on the particles on the differential front of each ray $\sRay$. Thus, if the probability of hitting a particle is stochastic, and perfectly random, then the attenuation of the ray is $\sAttenuation(\sExtinction \,t)=e^{-\sExtinction \,t}$. In contrast, in the case of negative correlation of the particles, then the particles never shadow each other, which means that all of them extinct and that the extinction process itself is deterministic. In that limit case of perfect negative correlation, the attenuation is perfectly linear, and takes the form $\sAttenuation(\sExtinction \, t) = \max(1-\sExtinction\,t, 0)$. In the following sections we stick to the random process, and use the exponential attenuation function. This means that although our radiative model (\Sec{ourgbe}) and our form of transmittance \ParEq{transmittance_general} are general, we limit our results to the case of positive correlation, which is more common in natural media. }

\subsection{Correlation between light and particles}
\new{An important aspect of \Eq{transmittance_general} is that it accounts for the distribution of intensity on along the light beam, as well as its relationship with the particles distribution. 
%
This allows to express the effect of boundary conditions as described in \Sec{boundary}, in particular in the media-to-media situation where the distribution of incoming light at the boundary $\sProbLight{\sRad_i}$ is dependent on the media traversed before reaching the boundary, and depending on its correlation with the next media's particles (modeled with the conditional probability $\sProbExtinctionConditional{\sExtinction}{\sRad_i}$) will have higher or lower probability of interaction. }

\new{Moreover, it implicitely models the different extinction probability existing between emitted and scattered light (\Sec{ourgbe}), since emitted light will likely be decorrelated from the particles (and thus $\sProbExtinctionConditional{\sExtinction}{\sRad_i} = \sProbExtinction{\sExtinction}$), while once it is scattered the independence between $\sProbLight{\sRad_i}$ and $\sProbExtinction{\sExtinction}$ might sometimes not exist. }
\adrianc{This is probably easier to see with a figure, but maybe the paper is now too crowded...?}

\new{In the following, we will assume that the incoming light is always decorrelated from the particles (i.e. $\sProbLight{\sRad_i}$$ and \sProbExtinction{\sExtinction}$ are independent). What this means is that incoming light is assumed to be uniformly distributed and, more importantly, although light becomes correlated with the media after scattering, we assume that this light distribution is decorrelated with the scattering of the next extinction event. Under this assumption, and imposing exponential attenuation, we transform \Eq{transmittance_general} to (see Annex XX)
%
\begin{align}
\sTranmittanceCorr(t) &= \int_0^\infty \,e^{-\sExtinction\,t}\sProbExtinction{\sExtinction}\diff{\sExtinction},
\label{eq:transmittance}
\end{align}
%
while the extinction probability $\sProb{t}$ is:
%
\begin{align}
\sProb{t} &= \int_0^\infty \,\sExtinction e^{-\sExtinction\,t}\sProbExtinction{\sExtinction}\diff{\sExtinction}.
\label{eq:pathlength}
\end{align}
%
Note that this form of $\sProb{t}$ is a generalization of the simple example modeled in \Eq{prob_two_extinction} to an arbitrary (continuous) mixture of extinction coefficients $\sExtinction$.}

\new{Interestingly, Davis and Xu~\shortcite{Davis2014Generalized} proposed a similar form for transmittance in correlated media, based on observations of transmittance in clouds. This makes perfect sense, since they only care about transmittance from an external light source uncorrelated with the medium, which presents a uniform distribution $\sProbLight{\sRad_i}$. 
%
Moreover, in their work, the authors state that the existence of an integro-differential counterpart of their derivation is unknown. 
By using \Eqs{pathlength}{extinctionresolved} this form of transmittance can be directly plugged into the extended GBE, under the assumptions discussed in the begining of the section. Therefore the GBE is in fact its integro-differntial form. We have thus offered a more general form of transmittance than Davis and Xu's, and linked these two complementary views of light transport in correlated media.}

\subsection{Optical Properties of Locally-Correlated Media}
\label{sec:optical_properties}

%\adrianc{Again, need to talk on how the $t$-dependent phase function $\sPF$ and scattering albedo $\sAlbedo$ are defined from a bulk of particles.}
\Eqs{integral_grte}{transmittance} model the appearance of the medium based on three main optical parameters: the albedo $\sAlbedo$, the phase function $\sPF$, and, different from the classic RTE \ParEqs{rte}{anisrte}, the probability distribution function of the extinction $\sProbExtinction{\sExtinction}$. 
%The first two ($\sAlbedo(\diro)$ and $\sPF(\diri,\diro)$) are defined as in \Eq{extinction_jakob}. 
%The only difference is the directional dependency of $\sProbConditional{\sConcentration}{\diro}$ in case of anisotropic media. 
%, which in the case of isotropic media the directional dependence disapears. 
\new{From the definition of extinction $\sExtinction$ in \Eq{extinction_jakob} we can define:
%
\begin{equation}
\sExtinction\,\sProbExtinction{\sExtinction}= \sConcentration\,\sProbConc{\sConcentration}\int_0^\infty\sCrossSection \sProbConditional{\sCrossSection}{\sConcentration} \diff{\sCrossSection}, 
\label{eq:isotropic_structure_correlation}
\end{equation}
%
where $\sProbConc{\sConcentration}$ is the probability distribution of the particles concentration and $\sProbConditional{\sCrossSection}{\sConcentration}$ is the conditional probability distribution between the cross section $\sCrossSection$ and the concentration $\sConcentration$. Assuming that these parameters are independent leads to an average constant cross section, which in turn yields: 
\begin{equation}
\sExtinction\,\sProbExtinction{\sExtinction}= \sConcentration\,\sProbConc{\sConcentration}\, \sCrossSection.
\label{eq:isotropic_structure}
\end{equation}
%
This formulation results into $\sProbExtinction{\sExtinction}\propto\sProbConc{\sConcentration}$, but imposes that $\sProbExtinction{\sExtinction}$ is independent of the cross section $\sCrossSection$. }

Physically, \Eq{isotropic_structure} models extinction based on the different concentrations of participating particles with an average cross section $\sCrossSection$ within a differential volume. 

%
%\adrianc{Add note on what this intuitively means, since it is important to explain later the integro-differential form. From~\cite{Larsen2011Generalized}``$\sExtinction\,\sProbExtinction{\sExtinction}$ is the probability (averaged over all physical realization) that a particle will experience a collision after traveling a distance $\sExtinction^{-1}$.'' In traditional transport, this averaged distance will always be $\Mean{\sExtinction}^{-1}$, with $\Mean{\sExtinction}=\int_0^\infty \sExtinction\,\sProbExtinction{\sExtinction} \diff{\sExtinction}$.}

We have so far assumed isotropy for both $\sProbConc{\sConcentration}$ and $\sCrossSection$. While this works well for media made up of spherical particles, as well as randomly correlated media (e.g. exhibiting fractal structure), other media present  anisotropic structure. 
%
By applying \Eq{isotropic_structure} to \Eq{extinction_jakob}, and considering the directional dependency of the probability distribution of the particles concentration $\sProbConditional{\sConcentration}{\diro}$, we get: 
%
\begin{align}
\sExtinction \sProbConditional{\sExtinction}{\diro} & = \sConcentration \sProbConditional{\sConcentration}{\diro} \int_\Sphere \sCrossSection(\diro,\dir)\sProbDir{\dir}\diff{\dir} \nonumber \\
& = \sConcentration \sProbConditional{\sConcentration}{\diro} \, \Mean{\sCrossSection}(\diro),
\label{eq:anisotropic_structure}
\end{align}
%
where $\Mean{\sCrossSection}$ is the mean cross section along $\diro$. Note that again we consider $\sConcentration$ and $\sProbDir{\dir}$ to be independent. \new{Finally, the remaining optical properties of the media encoded in the scattering operator $\sScatteringOperator(\px,\diri,\diro,t)$ can be computed trivially using \Eq{freepath_mixture}.}
%
%\Fig{angular_structure} shows the effect of the angular dependency of $\sProbConditional{\sConcentration}{\diro}$, for heterogeneous volumes of cloth at micron scale.
%

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Old text!
\new{Under this assumption, and introducing the additional constraint of the beam of light being uniformly distributed on its front of propagation, we can generalize the simple example modeled in \Eq{prob_two_extinction} to an arbitrary continuous of optical depths $\sOpticalDepth_t$, defining the probability of a path length $t$ as (note that we omit the spatial and directional dependence for clarity):}
%
%In addition, we would like to have a closed-form solution for $\sTranmittanceCorr(\px,\py)$. %Let us first define the probability of light interacting at distance $t$ from point $\px$ as
%\new{By inverting \Eq{extinctionresolved}, and generalizing \Eq{prob_two_extinction} as an integral of optical depths $\sOpticalDepth_t$, we can define the probability of a path length $t$ as} 
%
\begin{equation}
\sProb{t} \, = \, \sExtinctionResolved(t)\,e^{\int_0^t\sExtinctionResolved(s)\diff{s}} \, = \,  \int_0^\infty\frac{\diff{\sOpticalDepth_t}}{\diff{t}} \,e^{-\sOpticalDepth_t}\sProbExtinction{\frac{\diff{\sOpticalDepth_t}}{\diff{t}}}\diff{\sOpticalDepth_t},
\label{eq:prob_grte}
\end{equation}
%
where $\sOpticalDepth_t=\int_0^t\sExtinction(\px_s)\diff{s}$ is the optical depth for distance $t$, and $\sProbExtinction{\sOpticalDepth_t}$ is the probability of a light beam to traverse an optical depth $\sOpticalDepth_t$. %\adrianc{I'd probably need to bring back the spatial dependence to make sense on the $\frac{\diff{\sOpticalDepth_t}}{\diff{t}}$ thing.} 
Intuitively, this relates the path-length distribution, with the average of optical depths that a photon can pass through when traveling a distance $t$. 

Using the physical definition of transmittance, we define $\sTranmittanceCorr(\px,\py)$ as:
%
\begin{align}
\sTranmittanceCorr(\px,\py) & = 1-\int_0^t \sProb{s}\diff{s} \nonumber \\
& = 1 - \int_0^t \int_0^\infty\frac{\diff{\sOpticalDepth_s}}{\diff{s}} \,e^{-\sOpticalDepth_s}\sProbExtinction{\frac{\diff{\sOpticalDepth_s}}{\diff{s}}}\diff{\sOpticalDepth_s}\diff{s}.
\label{eq:transmittance_general}
\end{align}
%
with $t=\|\px-\py\|$. 
%While \Eq{transmittance_general} is significantly more complex than the definition of transmittance in \Eq{integral_grte}, it has major interesting consequence: 
%This definition has a major interesting consequence: 
Assuming homogeneous or locally-homogeneous media, where the spatial dependence of $\sExtinctionResolved(t)$ and therefore $\sOpticalDepth_t$ can be neglected, we can now formulate $\sOpticalDepth_t=\sExtinction\,t$, which transforms \Eq{transmittance_general} into: %\footnote{Note that we distinguish between the extinction \emph{with memory} $\sExtinctionResolved(t)$ (i.e. dependent on the distance previously traveled by light), and the common extinction parameter used in radiative transfer $\sExtinction$, which can be computed as a function of the particles' cross section and density. }:
%
\begin{align}
\sTranmittanceCorr(\px,\py) &= 1 - \int_0^t \int_0^\infty\sExtinction \,e^{-\sExtinction\,s}\sProbExtinction{\sExtinction}\diff{\sExtinction}\diff{s} \nonumber \\
&= \int_0^\infty \,e^{-\sExtinction\,t}\sProbExtinction{\sExtinction}\diff{\sExtinction}.
\label{eq:transmittance}
\end{align}
%
%
Interestingly, Davis and Xu~\shortcite{Davis2014Generalized} proposed a similar form for transmittance in correlated media, based on observations of light transport in clouds. In their work, the authors state that the existence of an integro-differential counterpart of their derivation is unknown. 
\new{However, by means of \Eq{prob_grte} we have shown that this form of transmittance is a particular case of extended GBE, under the assumptions discussed in the begining of the section, and therefore the GBE is in fact its integro-differntial form. We have thus linked these two complementary views of light transport in correlated media.}
\new{In fact, using \Eqs{prob_grte}{transmittance} we can define $\sExtinctionResolved(t)$ as a function of $\sProbExtinction{\sExtinction}$. We give more details for our particular model in \Sec{rendering}. }

%Interestingly, Davis and Xu~\shortcite{Davis2014Generalized} proposed a similar form for transmittance in correlated media based on observations of light transport in clouds, although they did not derive it from the GBE (\Eq{grte}). In fact, they did not explicitly answer the existence of an integro-differential counterpart of their derivation. We have thus linked two complementary views of light transport in correlated media. 

The main implication of \Eq{transmittance} is that it presents the transmittance $\sTranmittanceCorr(t)$ as the moment generating function\footnote{The \textit{moment generating function} (mgf) $\sMGFProb{t}$ of a pdf $\sProb{x}$ is  $\sMGFProb{t}=\int_{-\infty}^{\infty}\exp(tx)\sProb{x}dx$. Note that the mgf might not always exist; in such cases, it is possible to use the characteristic function $\sCFProb{t}$ of the pdf, which is defined as the inverse Fourier transform of the latter $\sCFProb{t}=\InverseFourier{\sProb{x}}$.} of $\sProbExtinction{-\sExtinction}$. This means that, for a number of extinction distributions, we can compute the transmittance in locally-correlated media using a closed form solution. 
%
Moreover, it leads to a simple definition of the optical properties of the media, directly related to the particles cross sections and concentration. 
\new{This definition has however some limitations: due to the underlying exponential in \Eq{prob_grte}, we are assuming that despite correlation, the process of extinction of a differential beam of light is still Poissonian. This makes perfect sense on positively correlated media, as well as uncorrelated media; however, such exponential fails to model faster-than-exponential extinction in negatively correlated media. Still, despite these limitations, the presented model is valid for a number of different media, as we will show in the following sections. } 
%Note that we have omitted anisotropy in our derivations, but this could be seamlessly added by introducing a directional dependence in $\sExtinctionResolved(t)$ and $\sExtinction$, as we show in the following. 


\adrianc{This is the original formulation that we submitted to SigAsia. It is correct under a bunch of assumptions, but the good thing is that has already been observed in real-world, and that gives reasonable good results under a reasonable set of assumptions, and now it's well related with the GBE (revs complaint about that in the first submission). However, it is limited by the assumptions: 
%
The first one (differential length of correlation) is intrinsic to this model, and cannot be avoided (basically, it assumes that the particles along the direction of propagation are randomly distributed). The second assumption (uncorrelated light wrt the particles) might be more important, and could be solved with some more mathematical complexity; the good thing of removing this second assumption is that we could easily include all other boundary conditions and particle-to-particle interactions would be more gracefully handled (right now, we should assume decorrelation between scattered light and particles, which is not the best-case scenario). Finally, the latter assumption (underlying Poissonian proccess avoiding negative correlation) would require changing the exponential decay in \Eq{prob_grte} by a linear one (perfect negative correlation) or a blend of both. 
%
In summary, I think now we address most previous concerns, and explicitly state the limitations and assumptions of our model, which is good. However, this could be extended to more diverse interactions, under a nicer mathematical framework with some little time. But first, let's get the paper done :).
}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Optical Properties of Locally-Correlated Media}
\label{sec:optical_properties}

%\adrianc{Again, need to talk on how the $t$-dependent phase function $\sPF$ and scattering albedo $\sAlbedo$ are defined from a bulk of particles.}
\Eqs{integral_grte}{transmittance} model the appearance of the medium based on three main optical parameters: the albedo $\sAlbedo$, the phase function $\sPF$, and, different from the classic RTE (\Eqs{rte}{anisrte}), the probability distribution function of the extinction $\sProbExtinction{\sExtinction}$. 
%The first two ($\sAlbedo(\diro)$ and $\sPF(\diri,\diro)$) are defined as in \Eq{extinction_jakob}. 
%The only difference is the directional dependency of $\sProbConditional{\sConcentration}{\diro}$ in case of anisotropic media. 
%, which in the case of isotropic media the directional dependence disapears. 
\new{From the definition of extinction $\sExtinction$ in \Eq{extinction_jakob}, and imposing that $\sProbExtinction{\sExtinction}\propto\sProbConc{\sConcentration}$, with $\sProbConc{\sConcentration}$ the probability distribution of the particles concentration,} we can define:
%
\begin{equation}
\sExtinction\,\sProbExtinction{\sExtinction}= \sConcentration\,\sProbConc{\sConcentration}\int_0^\infty\sCrossSection \sProbConditional{\sCrossSection}{\sConcentration} \diff{\sCrossSection}, 
\label{eq:isotropic_structure_correlation}
\end{equation}
%
where $\sProbConditional{\sCrossSection}{\sConcentration}$ is the conditional probability distribution between the cross section $\sCrossSection$ and the concentration $\sConcentration$. \adrianc{I'm sure that \Eq{isotropic_structure} holds, but as \RevTF asks, can \Eq{isotropic_structure_correlation} give the same $\sExtinction$ with different $\sConcentration$'s? I think it might, depending on $\sProbConditional{\sCrossSection}{\sConcentration}$. Check and revise if needed!} Assuming that these parameters are independent leads to an average constant cross section, which in turn yields: 
\begin{equation}
\sExtinction\,\sProbExtinction{\sExtinction}= \sConcentration\,\sProbConc{\sConcentration}\, \sCrossSection.
\label{eq:isotropic_structure}
\end{equation}
%
This formulation imposes that $\sProbExtinction{\sExtinction}$ is independent of the cross section $\sCrossSection$. Physically, \Eq{isotropic_structure} models extinction based on the different concentrations of participating particles with an average cross section $\sCrossSection$ within a differential volume. 

%
%\adrianc{Add note on what this intuitively means, since it is important to explain later the integro-differential form. From~\cite{Larsen2011Generalized}``$\sExtinction\,\sProbExtinction{\sExtinction}$ is the probability (averaged over all physical realization) that a particle will experience a collision after traveling a distance $\sExtinction^{-1}$.'' In traditional transport, this averaged distance will always be $\Mean{\sExtinction}^{-1}$, with $\Mean{\sExtinction}=\int_0^\infty \sExtinction\,\sProbExtinction{\sExtinction} \diff{\sExtinction}$.}

We have so far assumed isotropy for both $\sProbConc{\sConcentration}$ and $\sCrossSection$. While this works well for media made up of spherical particles, as well as randomly correlated media (e.g. exhibiting fractal structure), other media present  anisotropic structure. 
%
By applying \Eq{isotropic_structure} to \Eq{extinction_jakob}, and considering the directional dependency of the probability distribution of the particles concentration $\sProbConditional{\sConcentration}{\diro}$, we get: 
%
\begin{align}
\sExtinction \sProbConditional{\sExtinction}{\diro} & = \sConcentration \sProbConditional{\sConcentration}{\diro} \int_\Sphere \sCrossSection(\diro,\dir)\sProbDir{\dir}\diff{\dir} \nonumber \\
& = \sConcentration \sProbConditional{\sConcentration}{\diro} \, \Mean{\sCrossSection}(\diro),
\label{eq:anisotropic_structure}
\end{align}
%
where $\Mean{\sCrossSection}$ is the mean cross section along $\diro$. Note that again we consider $\sConcentration$ and $\sProbDir{\dir}$ to be independent. \new{Finally, the remaining optical properties of the media encoded in the scattering operator $\sScatteringOperator(\px,\diri,\diro,t)$ can be computed trivially using \Eq{freepath_mixture}.}
%
%\Fig{angular_structure} shows the effect of the angular dependency of $\sProbConditional{\sConcentration}{\diro}$, for heterogeneous volumes of cloth at micron scale.
%




\endinput

%%%% OLD SEC's INTRO
\Eqs{integral_grte}{integral_inscattering} define the media properties as average differential probabilities of extinction $\sExtinctionResolved(t)$ (or scattering $\sScatteringResolved(t)$), which are computed from the probability of extinction $\sProb{t}$ via \Eq{extinctionresolved}. 
%
Unfortunately, as opposed to classic light transport, this is not directly dependent on the primal optical properties of the media (e.g. the extinction coefficient $\sExtinction=\sConcentration\,\sCrossSection$). The main reason is the memory-effect associated to $\sExtinctionResolved(t)$, which does not only account for the local optical properties of the media but also for the path traversed beforehand. 
%
In fact, the usual approach is to precompute and tabulate the probability of extinction $\sProb{t}$~\cite{Moon2007Discrete,Larsen2011Generalized,Frank2010Generalized} via simulation.  
%
Instead, we want to define media properties based on commonly used media optical properties: particles density $\sConcentration$ and cross section $\sCrossSection$. This has obvious advantages to allow for more intuitive direct definition of the media, as well as editing its optical properties locally. 
} \adrianc{Maybe a table with the symbols we're using, their units, and what they mean in the RTE and S-RTE can be useful to further clarify what they mean and how they are different?}

%Defining the media properties as the mean probability of extinction for light paths of length $t$ is not intuitive. In fact, the most common approach is to precompute and tabulate the path-length dependent extinction, assuming statistically homogeneous media~\cite{Larsen2011Generalized,Frank2010Generalized}. 
%
%Unfortunately, this does not have a direct relationship with the definition of the optical properties of the medium, as is common in graphics. Moreover, this definition implies two additional integrals that need to be evaluated numerically, even in homogeneous media. 
%
%\adrianc{Something interesting of this section is that we are assuming that the distance between particles is very small (within a differential of length $dt$). This makes sense considering that we are talking about \emph{"differential volumes"}. With that in place, we can articulate all description done here, which is a particular case of the G$^2$BE described before, in which the probability of extinction $p(t)$ is always decreasing. If there were the case of a distance to scatterers larger than $dt$, then $p(t)$ could have, and in fact it does, a global maxima with $dp(t)/dt = 0$. But with that assumption this problem is eliminated. }


\new{In order to do so, let us return to the description of the effect of correlation over extinction (\Sec{correlation}), and in particular on how that effect is illustrated in \Fig{kostinskis}: When light traverses a correlated medium it is attenuated differently depending on the distribution of particles. Let us assume that correlation occurs in a differential volume, and thus the scale of correlation is smaller than a differential distance $\diff{t}$: this assumption is important, since imposes that the travel distance is always larger than the distance between particles. This is not the case for e.g. particlate media~\cite{Moon2007}, where the explict path length distribution needs to be used (instead of one derived from the optical properties of the media). Despite this limitation, as we will see it will allow for a simpler definition of the media, which is still general enough for graphics applications. 
}
%%%% OLD SEC's INTRO





Alternatively, we can formulate $\sProb{t}$ as:
\begin{align}
\sProb{t} = \left| \frac{\diff{\sTranmittanceCorr(t)}}{\diff{t}} \right| \, \rightarrow \, \sTranmittanceCorr(t) = - \int_0^t \sProb{s}\diff{s}.
\end{align}
%
By integrating the second equality in \Eq{prob_grte}, we can formulate the transmittance in correlated media as a distribution of optical depths:
\begin{equation}
\sTranmittanceCorr(\px,\py) = \int_0^\infty\Exp{-\sOpticalDepth}\sProb{\sOpticalDepth}\diff{\sOpticalDepth},
\label{eq:correlated_transmittance}
\end{equation}



However, as shown by Davis and Marshak~\shortcite{Davis2004Photon}, we can define the integral form of the RTE (\Eq{integral_grte}), and in particular the transmittance term, as a distribution of the medium optical depths $\sOpticalDepth$. This transforms the transmittance $\sTranmittanceCorr(\px,\px_t)$ in \Eq{integral_grte} to:
%
\begin{equation}
\sTranmittanceCorr(\px,\py) = \int_0^\infty\Exp{-\sOpticalDepth}\sProb{\sOpticalDepth}\diff{\sOpticalDepth},
\label{eq:correlated_transmittance}
\end{equation}
%
where $\sProb{\sOpticalDepth}$ is the probability of optical depth $\sOpticalDepth$. \adrianc{There were no proof of equivalence between both approaches (in fact, \cite{Davis2014Generalized} hypothesized on the lack of an integro-differential form of \Eq{correlated_transmittance}. But I think I have proven they are equivalent, at least for the homogeneous case. For the heterogeneous, I'm still a bit worried (see previous comment).} Putting transmittance, and therefore \Eq{integral_grte} in this form does not only allow to relate the optical properties of the media with the transmittance directly, but also to compute efficiently the transmittance, as we will show in the previous sections. We first will demonstrate the implications of light transport in correlated media in statistically homogeneous  media, and then generalize to heterogeneous media. 


\endinput
\section{Radiative Transport in Locally Structured Media}
\label{sec:volumetric}

The formulation of the RTE, as described before, assumes that the position of the particles in a differential volume is random and perfectly decorrelated. In practice, this means that there is the probability of interacting with a participating particle is uniform along the differential volume, and thus any possible source of heterogeneity is at macroscopic level. However, in practice that is not true except at very fine scale. 

\adrianc{To be fair, we should acknowledge early works of Lovejoy, who described the effects of correlated media in the late 80s and early 90s, by studying the fractal structure of clouds. }
Taking clouds as example, the aerosol particles forming the cloud tend to form clusters, which results in areas with higher optical thickness, and even empty areas at different scale levels~\cite{Marshak1998}. Kostinski~\shortcite{Kostinski2001Extinction} showed that the exponential attenuation predicted by the Beer-Lambert law does not hold in the presence of spatial structure; transmittance decays at a slower rate, following a long-tail distribution. 
%
This effect has also been observed in other structured media, such as trees~\cite{Knyazikhin1998}, closely packed particulate media~\cite{Peltoniemi1992}, and porous~\cite{Bellet2009,Taine2010} and fibrous media~\cite{Coquard2006}.

Highly structured volumetric media have been studied in computational transport outside computer graphics, in fields such as nuclear engineering~\cite{Levermore1986Linear,Larsen2011Generalized}, or atmospheric sciences~\cite{Newman1995Systematic,Davis1999Horizontal,Davis2004Photon}, leading to \textit{non-classical transport} theories~\cite{Larsen2007Generalized,Frank2010Generalized}. \adrianc{Rewrite! Same as in RW! Also, all sound so redundant...}
%
We leverage advances in those fields, and present in the following a new formulation of the radiative transfer equation (RTE)~\cite{Chandrasekhar1960}, which takes into account the effect of \textit{locally structured} media. Later, we combine it with Jakob et al.'s~\shortcite{Jakob2010Radiative} anisotropic RTE.
%Note that this formulation is orthogonal to the anisotropic RTE proposed by Jakob et al.~\shortcite{Jakob2010Radiative}, and hence can be included seamlessly into their model, as we show in \Sec{statmodel}. 
%%
%\DIEGO{Probably not here anymore, if we move it to implementation (cut?)} We then describe how this formulation is used to render our fiber-based volumetric description of cloth. 


\subsection{Modeling Local Structure}
As discussed in \Sec{background}, classical RTE assumes that a medium is locally homogeneous, in the sense that the probability of a beam of light to be attenuated (absorbed or scattered) is uniform in a differential volume around point $\px$. This is modeled using a uniform extinction coefficient $\sExtinctionResolved$. \adrianc{I feel I'm being extremely redundant, I think I've said this in every fuckin' section before this... Anyway, I'll clean that with a full read of all sections. }
%
However, this homogenization fails on modeling the small scale structure in a differential volume present in many media. One alternative would be to explicitly model this structure \adrianc{Wojciech did something similar to this in this papers of granular media}, but this could be prohibitively expensive. Instead, we take into account this variability by statistically modeling the extinction suffered by light due to correlation on the position of the particles, where higher correlation means more packed particles clustering. 

Instead of considering a single mean extinction value, we follow previous work on transport~\cite{Larsen2007Generalized,Davis2014Generalized} and assume a probability distribution of extinction coefficients $\sProbExtinction{\sExtinctionResolved}$. 
%
Intuitively, this means that at certain areas of the differential volume it is more probable to interact with the medium than at others. Assuming that the cross section remains constant, we model 
\begin{equation}
\sExtinctionResolved\,\sProbExtinction{\sExtinctionResolved}= \sConcentration\,\sProbConc{\sConcentration}\sCrossSection, 
\label{eq:isotropic_structure}
\end{equation}
with $\sProbConc{\sConcentration}$ the probability distribution of particles concentration. Note that this formulation means that $\sProbExtinction{\sExtinctionResolved}\propto\sProbConc{\sConcentration}$, and therefore is independent on the cross section $\sCrossSection$.
%
%\adrianc{Add note on what this intuitively means, since it is important to explain later the integro-differential form. From~\cite{Larsen2011Generalized}``$\sExtinctionResolved\,\sProbExtinction{\sExtinctionResolved}$ is the probability (averaged over all physical realization) that a particle will experience a collision after traveling a distance $\sExtinctionResolved^{-1}$.'' In traditional transport, this averaged distance will always be $\Mean{\sExtinctionResolved}^{-1}$, with $\Mean{\sExtinctionResolved}=\int_0^\infty \sExtinctionResolved\,\sProbExtinction{\sExtinctionResolved} \diff{\sExtinctionResolved}$.}

This formulation assumes isotropy on both $\sProbConc{\sConcentration}$ and $\sCrossSection$. While this works well for transport in media with spherical particles and randomly correlated media (e.g. exhibiting fractal structure), it might not be enough for more structured anisotropic media used in graphics. 
%
We generalize this formulation in two ways: On one hand, the spatial correlation in structured media might have different effects depending on the light direction $\diro$, making $\sProbConc{\sConcentration}$ directionally dependent, as exampled in \Fig{anisotropic_structure}\adrianc{This figure will show the effect of directionality on the angular extinction having an structured media (e.g. one with a well defined planar pattern)} \adrianc{Also, note that the angular dependence is also considered by Vasques and Larsen~\shortcite{Vasques2014AnisotropicTheory,Vasques2014AnisotropicApplication}; however, their definition is purely theoretical: while here we explain an actual form of doing this, combined with Jakob's anisotropic cross section they just do is to say: ``Hey, you can have some angular dependence''. } 
On the other, the cross section is directionally dependent in anisotropic media \Eq{extinction_jakob}. With these two forms of directional anistropy, we model  $\sExtinctionResolved\sProbExtinction{\sExtinctionResolved,\diro}$ as:
\begin{equation}
\sExtinctionResolved \sProbExtinction{\sExtinctionResolved,\diro} = \sConcentration \sProbConc{\sConcentration,\diro} \int_\Sphere \sCrossSection(\diro,\dir)\sProbDir{\dir}\diff{\dir}.
\label{eq:anisotropic_structure}
\end{equation}
For simplicity we are assuming no correlation between $\sProbConc{\sConcentration,\diro}$ and $\sProbDir{\dir}$, as well as uniform $\sCrossSection(\diro,\dir)$ in the differential volume. It is important to note that the spatial correlation in the particles position is assumed locally at a differential volume, and thus a medium can be still considered \emph{statistically homogeneous}, meaning that its statistically moments are invariant. 


The consequence of the non-uniformity in \Eqs{isotropic_structure}{anisotropic_structure} is that, even for statistically homogeneous media and differential propagation length, is that the probability of extinction is dependent on the distance flight by light from the previous interaction $t$. As such, we can consider that the extinction coefficient is dependent on $t$, and can define $\sExtinctionResolved(t,\diro)$ as the averaged differential probability that a photon will be extincted after traveling a distance $t$ in direction $\diro$~\cite{Larsen2011Generalized,Vasques2014AnisotropicTheory}. In the following we use this definition to introduce a generalized structured integro-differential form of the RTE; later we show how it relates with the more practical definition in \Eqs{isotropic_structure}{anisotropic_structure}.



\subsection{Structured RTE}
\adrianc{When writing this I was thinking on going from isotropic to anisotropic light transport; thus, I've written all in isotropic form, planning to generalize to its anisotropic form. But maybe is too much. One option would be to put at the end the anisotropic form, and then refer to an Annex for the ``we go from A to B''. Anyway, I haven't written anything about anisotropic media yet, until I have opinion.}
Once we have defined how to statistically model the structure within a differential volume, we can now redefine the transport equation ruling light transport. Assuming an isotropic structure (i.e. with no angular dependence, \Eq{isotropic_structure}), we transform \Eq{rte} into the \emph{Generalized Boltzmann Equation}~\cite{Larsen2007Generalized,Larsen2011Generalized}:
%
\begin{multline}
\frac{d}{dt}\sRad(\diro,t) + \diro\cdot\Diff{\sRad(\diro,t)} + \sExtinctionResolved(t)\sRad(\diro,t) = 0, \\
\sRad(\diro,0) = \int_0^\infty\sScattering(t)\int_\Sphere \sRad(\diri,t)\sPF(\diri,\diro)\diff{\diri}\diff{t} + \sEmission(\diro),
\label{eq:grte}
\end{multline}
%
with $\sScattering(t)=\sAlbedo\,\sExtinctionResolved(t)$ the probability of a particle to be scattered after traveling a distance $t$, and $\sRad(\diro,t)$ the radiance at $\px$ having traveled exactly $t$. 
The second line of the equation is the initial value for $t=0$ i.e. where light has zero distance from the last scattering event. Intuitively, this form of the Bolzmann equation assumes memory on the particle transport, which is reset when a scattering event is produced or emitted (at $t=0$). This memory effect, resulting on a dependence of the total traveled path $t$, is the main difference with respect to \Eq{rte}. Note that by removing the path-length dependence of the extinction as $\sExtinctionResolved(t) = \sExtinctionResolved$, and integrating \Eq{grte} with respect to $t$ between 0 and $\infty$ we get the classical RTE (\Eq{rte}).

%
While in graphics there are a few works solving the RTE in its differential form~\cite{Gutierrez2005,Munoz2014,Ament2014}, it is generally evaluated in its integral form. Generalizing Larsen and Vasques's integral definition~\cite{Larsen2011Generalized} to support heterogeneous media, we solve the Ordinal Differential Equation (ODE) defined in \Eq{grte} for the radiance incoming at point $\px$ \adrianc{I'd like to revise this once more: \cite{Larsen2011Generalized} modeled only their equation for homogeneous media, as well as others such as Davis~\cite{Davis2004Photon,Davis2014Generalized}. I have the (internal) proofs for the homogeneous case; but I'd like to be sure that this heterogeneous formulation is rock solid...}. 

%
\begin{equation}
\sRad(\diro) = \int_0^\infty \underbrace{e^{-\int_{0}^{t}\int_{0}^{t'}\sExtinctionResolved(\px_{t'},s)\diff{s}\diff{t'}}}_{\sTranmittanceCorr(\px,\px_t)} (\sRadICorr(\px_t,\diro) + \sEmission(\px_t,\diro))\diff{t},
\label{eq:integral_grte}
\end{equation}
%
where $\px_t = \px - \diro\,t$, $\sExtinctionResolved(\px_{t},s)$ is the probability of light having traveled a distance $s$ being extincted at point $\px_t$, and $\sTranmittanceCorr(\px,\px_t)$ is the transmittance between points $\px$ and $\px_t$. Finally, the inscattering $\sRadICorr(\px_t,\diro)$ at point $\px_t$ is
%
\begin{equation}
\sRadICorr(\px_t,\diro) = \int_0^\infty\sScattering(\px_t,t')\int_\Sphere \sRad(\px_{t'},\diri)\sTranmittanceCorr(\px_t,\px_{t'})\sPF(\diri,\diro)\diff{\diri}\diff{t'}.
\end{equation}
%

Unfortunately, defining the media properties for their use in \Eq{integral_grte} is not straight forward, and does not have a direct relationship with the physical definition of the medium optical properties described in \Eqs{isotropic_structure}{anisotropic_structure}. In fact, the approach generally followed in most previous work on non-classical transport (e.g. \cite{Larsen2011Generalized,Frank2010Generalized}) is to precompute and tabulate the path-length dependent extinction assuming an statistically homogeneous media. However, as shown by Davis and Marshak~\shortcite{Davis2004Photon}, we can define the integral form of the RTE (\Eq{integral_grte}), and in particular the transmittance term, as a distribution of the medium optical depths $\sOpticalDepth$. This transforms the transmittance $\sTranmittanceCorr(\px,\px_t)$ in \Eq{integral_grte} to:
%
\begin{equation}
\sTranmittanceCorr(\px,\py) = \int_0^\infty\Exp{-\sOpticalDepth}\sProb{\sOpticalDepth}\diff{\sOpticalDepth},
\label{eq:correlated_transmittance}
\end{equation}
%
where $\sProb{\sOpticalDepth}$ is the probability of optical depth $\sOpticalDepth$. \adrianc{There were no proof of equivalence between both approaches (in fact, \cite{Davis2014Generalized} hypothesized on the lack of an integro-differential form of \Eq{correlated_transmittance}. But I think I have proven they are equivalent, at least for the homogeneous case. For the heterogeneous, I'm still a bit worried (see previous comment).} Putting transmittance, and therefore \Eq{integral_grte} in this form does not only allow to relate the optical properties of the media with the transmittance directly, but also to compute efficiently the transmittance, as we will show in the previous sections. We first will demonstrate the implications of light transport in correlated media in statistically homogeneous  media, and then generalize to heterogeneous media. 







